Fair Allocation of Indivisible Items With Externalities

One of the important yet insufficiently studied subjects in fair allocation is the externality effect among agents. For a resource allocation problem, externalities imply that a bundle allocated to an agent may affect the utilities of other agents. In this paper, we conduct a study of fair allocation of indivisible goods when the externalities are not negligible. We present a simple and natural model, namely \emph{network externalities}, to capture the externalities. To evaluate fairness in the network externalities model, we generalize the idea behind the notion of maximin-share ($\MMS$) to achieve a new criterion, namely, \emph{extended-maximin-share} ($\EMMS$). Next, we consider two problems concerning our model. First, we discuss the computational aspects of finding the value of $\EMMS$ for every agent. For this, we introduce a generalized form of partitioning problem that includes many famous partitioning problems such as maximin, minimax, and leximin partitioning problems. We show that a $1/2$-approximation algorithm exists for this partitioning problem. Next, we investigate on finding approximately optimal $\EMMS$ allocations. That is, allocations that guarantee every agent a utility of at least a fraction of his extended-maximin-share. We show that under a natural assumption that the agents are $\alpha$-self-reliant, an $\alpha/2$-$\EMMS$ allocation always exists. The combination of this with the former result yields a polynomial-time $\alpha/4$-$\EMMS$ allocation algorithm.

==> conclusion.tex <==
An exciting open direction is to find approximation allocation algorithms for the general externalities model, with no restriction on the value of $\valu_{j,i}(\{\ite_k\})$. Many issues complicate the study of the general model. For example, the approximation algorithm presented for computing the value of $\EMMS_i$ is no longer applicable to this model. A good starting point is to study the general model for the cases with a few number of agents, e.g., 3 or 4 agents. 

For the network externalities model, one can think of improving the approximation ratio of the allocation. In particular, it would be interesting to propose an allocation algorithm with approximation factor independent of the self-reliance of the agents.

Another interesting open direction that might be of independent interest is to find a maximum value $\beta$, such that there exists a partition $P$ of the items in which $\worst_i(P)$ is a $\beta$-approximation of $\worst_i(O_i)$ for every agents $i$. Note that if such a partition exists, any allocation of it to the agents is a $\beta$-$\EMMS$ allocation.


Finally, it is very impressive to present a $PTAS$ for finding the optimal partition for an agent in the network externalities model. As said before, the ideas in \cite{woeginger1997polynomial} can not be directly applied to this problem.




